SpeechPrompt v2: Prompt Tuning for Speech Classification Tasks

Prompt tuning is a technology that tunes a small set of parameters to steer a pre-trained language model (LM) to directly generate the output for downstream tasks. Recently, prompt tuning has demonstrated its storage and computation efficiency in both natural language processing (NLP) and speech processing fields. These advantages have also revealed prompt tuning as a candidate approach to serving pre-trained LM for multiple tasks in a unified manner. For speech processing, SpeechPrompt shows its high parameter efficiency and competitive performance on a few speech classification tasks. However, whether SpeechPrompt is capable of serving a large number of tasks is unanswered. In this work, we propose SpeechPrompt v2, a prompt tuning framework capable of performing a wide variety of speech classification tasks, covering multiple languages and prosody-related tasks. The experiment result shows that SpeechPrompt v2 achieves performance on par with prior works with less than 0.15M trainable parameters in a unified framework.

==> 5_result_old.tex <==
% \input{assets/learnable_verbalizer_analysis_table}
\subsection{Speech Classification}
Table \ref{main_result} shows the result of SpeechPrompt v2 (GSLM+ and pGSLM+) on a wide variety of speech processing tasks. 
%
We show that when using either GSLM or pGSLM as the backbone spoken LMs, SpeechPrompt v2 achieves competitive performance on all content-related speech classification tasks. 
%
On the other hand, SpeechPrompt v2 can also generalize well across different languages, as we achieve new state-of-the-art results on low-resource Lithuanian SC and Arabic SC~\cite{DBLP:journals/corr/abs-2110-03894}.
%
Our framework falls slightly behind the prior works for prosody-related tasks but is still competitive. We find that with prosody informed, pGSLM outperforms GSLM in most prosody-related tasks, demonstrating the necessity of diverse spoken LMs for downstream tasks with different properties.
%
However, we can observe that the prompting method does not perform well for more challenging tasks (FSD and ER), where both content and prosody information must be considered simultaneously.
%
Moreover, our framework fails to perform well on the audio classification task (AuC) but achieves a comparable result on VAD. We argue that the spoken LMs cannot properly model the non-speech information but are still capable of separating the speech and non-speech patterns.
%
The result also shows that, empirically, using a learnable verbalizer in our framework steadily improves the performance, which indicates alleviating the information loss problem in the unit-to-class mapping process.
%
Overall, SpeechPrompt v2 demonstrates competitive results on various speech classification tasks, and the learnable verbalizer improves performance in most cases. Following, we further analyze the behavior of the verbalizer to get more insight into the label mapping process in prompting for speech processing.

\

\begin{figure}[t]
    \centering
    \subfloat[Class ``YES'']{
        \includegraphics[width=\linewidth]{assets/analyzing_verbalizer_class_yes.pdf}
    }
    
    \subfloat[Class ``LEFT'']{
        \includegraphics[width=\linewidth]{assets/analyzing_verbalizer_class_left.pdf}
    }
    \caption{The SHAP analysis of the learnable verbalizer on the Google Speech Command dataset~\cite{vygon2021learning}. Each point refers to one datapoint.} %For each chart, the horizontal axis is the SHAP value, while the vertical axis indicates the order of importance of each unit to the class from top to bottom. Each point refers to one datapoint.}
    \label{fig:analyzing_verbalizer}
    \vspace{-15pt}
\end{figure}

\vspace{-0.5em}
\subsection{Learnable Verbalizer Analysis}
% According to the experiment results, the proposed learnable verbalizer considerably improves the performance in most tasks. 
In this section, we further inspect the behavior of the learnable verbalizer to see how it maps the discrete units to meaningful task labels. Specifically, we adopt Shapley Additive exPlanation~\cite{lundberg2017unified} (SHAP), a popular method to interpret model predictions. In SHAP, the \textbf{SHAP value} is calculated to measure the importance of each input feature, here referring to the discrete unit, to a single prediction made by the model. 

Fig.\ref{fig:analyzing_verbalizer} shows the result of SCR on Google SC dataset for three different runs. We list the top 10 units contributing to the class ``YES'' and the class ``LEFT'' 
\footnote{Please refer to our project website for more demonstration. \url{https://ga642381.github.io/SpeechPrompt}}.
In each chart, the horizontal axis is the SHAP value, while the vertical axis indicates the order of importance of each unit from top to bottom. 
Each point refers to the interpretation of a single datapoint. The color of a point reflects the magnitude of the value for each input unit.
% According to the experiment results, we can observe that the learnable verbalizer considerably improves the performance in most of the cases. However, it is still obscure why the proposed verbalizer is able and how it maps the discrete phonetic units to meaningful class labels. In this section, we further inspect its behavior to gain a deeper insight, and also to see whether the behavior remains consistent with different random seeds. We utilize Shapley Additive exPlanation~\cite{lundberg2017unified} (SHAP), a popular method to interpret model predictions. Inspired by Shapley Value in cooperative game theory~\cite{RM-670-PR}, given a single prediction, SHAP calculates the SHAP value for each input feature and therefore telling how important each feature is. Figure~\ref{fig:analyzing_verbalizer} shows the results on Google Speech Command Dataset for 3 different runs\footnote{Due to space limitations, we only list the top-10 units contributing to the class "yes" and "left". Please refer to our website for detailed demonstration}. 
% For each chart, the horizontal axis is the SHAP value while the vertical axis indicates the order of importance of each unit to the class from top to bottom. Each point refers to the interpretation of a single datapoint.
First, we observe that even in the same class, the importance of each unit varies from prediction to prediction. And the learnable verbalizer relies on multiple units to determine the output, indicating a many-to-many mapping behavior from units to labels. This verifies the possible information loss in the previous work, as described in sec\ref{sec:learnable_verbalizer}.
Moreover, the relationship between units and labels does not remain consistent in different runs. 
However, there are units in common and their contribution pattern is similar in different runs (e.g. unit 98 has the same pattern for class ``YES'').
%However, some common points do exist, and the way how a unit contributes seems to be definite (e.g. unit 98 for class ``YES'', unit 43 for class ``LEFT''). 
Last, the learnable verbalizer might use one unit to separate different classes. For example, when unit 98 has a lower value, the verbalizer is more likely to predict class ``LEFT'' instead of class ``YES''.
Overall, the analysis suggests that using a learnable verbalizer offers benefits over naive random mapping and frequency-based mapping and is more ideal for our framework. 


%\input{assets/learnable_verbalizer_analysis_table}

% Unlike the Language Model in NLP, the vocabulary in the spoken language model is not intuitive. For text classification in NLP, for example, to classify a document into several categories, the word of the category itself can be served as the prediction target of the LM's output. However, the output of the spoken language models is pseudo units and prosody information, which are low-level information of an utterance. To this end, a verbalizer is more important to the spoken language model than to the normal LM to achieve promising performances.

% In this work, we propose a learnable verbalizer on top of the spoken language models to alleviate the issue that the output of the spoken language model does not contain high-level meaning. We would like to emphasize that adopting a neural network as the verbalizer is not an originality in this work. Previous works also explore using classification heads to predict the output for downstream tasks. We are the first ones to point out the fundamentally different role of the verbalizer to the spoken language model an normal language model.
% [2022/10/13 03:15] Wei-Cheng's template below
% We first plot out the visualization of the mapping from unit to task label. [put some results here....]

% Moreover, we also find out that [some findings to support the upper visualization....]

% We also inspect how the number of unit affect the effectiveness of the learnable verbalizer. When we varies the number of unit available, the performance [blah blah blah...]

% Overall, we can conclude that the learnable verbalizer is necessary for our framework.





% Some plans about the verbalizer below

% * Different from NLP:
%     1. the units are not meaningful
%     2. the vocabulary size is relative small. For tasks with many classes, learnable verbalizer is necessary

% * What's the learned mapping 
%     1. the relation of the units and the task labels
%     2. one-to-one mapping?
%     3. many-to-one mapping?

% * Is there a set of units suitable for classification tasks and why?
%     e.g., unit 1, 2, 3, 4, ... are all important in the linear verbalizer across tasks

% * Unit space and the importance of learnable verbalzier
%     50 units performance gain
%     100 units performance gain
%     200 units performance gain

% \hua{Complementary - Possible Analysis:
% 1. mapping visualization;
% 2. sequence distribution change visualization; (if applicable --> end-task labels have sequence?)
% 3. hyper-parameter performance table (hyper-params include dropout, temperature, bias=True/False);
% 4. Error Analysis. 
% }
% Same Google Slide for detail: https://docs.google.com/presentation/d/1V52wKqX3L5GRHy30b0l3bPiCa4GVe4I1wkorznzYL2I/edit?usp=sharing

